Alpha Invariance: On Inverse Scaling Between Distance and Volume Density in Neural Radiance Fields

Scale-ambiguity in 3D scene dimensions leads to magnitude-ambiguity of volumetric densities in neural radiance fields, i.e., the densities double when scene size is halved, and vice versa. We call this property alpha invariance. For NeRFs to better maintain alpha invariance, we recommend 1) parameterizing both distance and volume densities in log space, and 2) a discretization-agnostic initialization strategy to guarantee high ray transmittance. We revisit a few popular radiance field models and find that these systems use various heuristics to deal with issues arising from scene scaling. We test their behaviors and show our recipe to be more robust.

==> rebuttal.tex <==
We thank the reviewers for their encouraging comments and constructive feedback. 
We have incorporated the writing/typo suggestions in our updated draft, and have included a more polished version of the pseudo-code in the main text.





\noindent\textcolor{mypurple}{\hrulefill ~~ \bf To Reviewer GDFv ~~ \hrulefill }

\question{mypurple}{
Explanation of $\alpha$ in Equation 2.
}{}
\answer{
We will make the transition from continuous integration to discrete $\alpha$-compositing clearer in the main text.
}

\question{mypurple}{
 High transmittance initializations for other activation functions. 
}{}
\answer{
It is significantly harder to write down closed form formulae for high transmittance initialization in the case of $\mathtt{relu}$ and $\mathtt{softplus}$.
We could attempt it using Monte Carlo estimates of their mean. Recall our goal is to achieve $\E[\sigma] \cdot L = \log(\frac{1}{T'})$. Assuming the pre-activation neural field output is drawn from $\mathcal{N}(0, 1)$, the expectations of the post-activation random variables can be approximated by sample mean. When $T'=0.99$, the RHS is $0.001$. We want to \emph{avoid} directly scaling down density or L to meet this target, since that would make it even harder for $\mathtt{relu}$ and $\mathtt{softplus}$ to achieve large density needed at solid regions. Instead the low transmittance should be achieved by shifting the activation function profile to the right, i.e. adding negative offset to the input. The correct offset can be tuned numerically. 
This procedure is significantly more tedious than the closed-form formula for $\mathtt{exp}$ activation, where we take advantage of the fact that scaling on the outside can be absorbed as offset on the input argument. 



\noindent\textcolor{myblue}{\hrulefill ~~ \bf To Reviewer mVZb ~~ \hrulefill }

\question{myblue}{
$w(t)$ and the derivative of $1-T(t)$.
}{}
\answer{
$(1-T(t))' = \frac{d}{dt} (- \exp(-\int_0^t \sigma(s) \, ds)) = -\sigma(t) \cdot -\exp(-\int_0^t \sigma(s) \, ds) = \sigma(t)\,T(t) = w(t) $. 
As described in lines 558-564 of the appendix, this is a restatement of the exponential distribution. 
We will incorporate this discussion in the main text. 
}

\question{myblue}{Plenoxels CDF Plot.}
\answer{
In Figure 5, $k$ is kept at $1.0$. Instead of analyzing Plenoxels' robustness to various scene scales, we ablate Plenoxels' design choice of using an unusually large initial learning rate of $30.0$ on the volumetric densities to achieve convergence.
We find that reducing this learning rate prevents the model from learning the correct numerical range on $\sigma$, and is directly correlated with poor convergence and rendering quality, as shown in Table 5.
}

\noindent\textcolor{myorange}{\hrulefill ~~ \bf To Reviewer  KsWp ~~ \hrulefill }


\question{myorange}{
    Clarification on Sampling Strategy and Experiment Protocol. 
}{}
\answer{
In lines 225-226, we describe that ``we leave the rest of the optimization hyperparameters such as sampling strategies unchanged.'' 
By sampling strategy, we mean the number of samples and the distribution of samples along each ray. Hence when we vary $L$, the sample spacing is increased/decreased proportionately. This keeps the relationship between
ray segment length and local opacity the same, and isolates the ability of the 
underlying neural field to predict densities at the correct magnitude. 
Our experiments show that using both $\exp$ and our high transmittance initialization
are needed to achieve robust performance w.r.t. scene scaling. 
We will revise the draft to further clarify this protocol.
}


\question{myorange}{
``Changing the scene scale by a large factor on inward-facing (object-level) scenes with known camera poses may not be that practical. Scene bounds are typically defined by the (known) camera poses.''
}{}
\answer{
Given a set of images, solving for their poses using SfM / V-SLAM runs into the ambiguity of relative camera translation. A common practice is to set the distance between the first camera pair to 1, and it results in the overall ambiguity of scene size. \textbf{This is a critical property of 3D reconstruction, and a fundamental motivation for our work}. 
It applies to inward-facing, object-centric scenes. 
Even with hardware distance measurements, there is an ambiguity in the physical units: meters, feet, or yards. The fact that the original NeRF authors set the radius for blender scenes to $4.0$ doesn't prevent us from switching to a different ruler.
}


\question{myorange}{
Empirical evidence and theoretical explanation for the advantages of $\exp$.
}{}
\answer{
As described in lines 75-77, 
our method brings consistent performance across various scene scalings. 
We believe that our experiments provide comprehensive evidence that using $\exp$ activation and our high transmittance initialization are critical for maintaining alpha invariance. 
Our results in Tables 2, 4, 5, 6, A1, and A2 show that regardless of the density encoding (MLP, voxel, and MLP/hashgrid hybrid) and scene type (synthetic, forward-facing, unbounded inward-facing, and indoor), our two-step method enables consistent convergence across all scene scales, while the baseline architectures exhibit many failure modes. 
For a more theoretical explanation, refer to Figure 2; when parameterizing $\sigma$ with $\mathtt{relu}$ or $\mathtt{softplus}$, the transitions from low-to-high $\alpha$ values are abrupt whereas $\exp$ provides smooth transitions across all $d$.




}





\noindent\textcolor{mygreen}{\hrulefill ~~ \bf To Reviewer NNdx ~~ \hrulefill }

\question{mygreen}{
TensoRF and DvGO.
}{}
\answer{
TensoRF uses a fixed distance scaling of $25.0$.
At $k=0.1$, the model fails to converge since the underlying $\mathtt{softplus}$ activation struggles to produce large sigmas at small distance scalings. 
DvGO creates a canonical scene size based on the voxel grid resolution, and not the physical ray length $L$. Since the focus of our study is robustness to scene scale, we tested DvGO's ability to handle further rescaling on this canonical scene size and observe that it also fails at small $k$ because $\mathtt{softplus}$ struggles at small distance scalings.
}













}




